Results of the Survey on the Future of HEP

The Young Physicists Panel (YPP) summarizes results from their Survey on the Future of High Energy Physics, which was conducted from July 2 to July 15, 2001. Over 1500 physicists from around the world, both young and tenured, responded to the survey. We first describe the origin, design, and advertisement of the survey, and then present the demographics of the respondents. Following sections analyze the collected opinions on the desire for balance in the field, the impact of globalization, the necessity of outreach, how to build the field, the physics that drives the field, and the selection of the next big machine. Respondents' comments follow the survey analysis in an appendix.

==> abstract2.tex <==
\begin{center}
\vspace*{.2 in}
{\large \bf ABSTRACT\\}
\vspace*{.5 in}
\end{center}

\vspace{0.5 in}
The Young Physicists Panel (YPP) summarizes results from
their \textit{Survey on the Future of High Energy Physics}, which was conducted
from July 2 to July 15, 2001. Over 1500 physicists from around the world, both
young and tenured, responded to the survey. We first describe the origin, design, 
and advertisement of the survey, and then present the demographics of the
respondents. Following sections analyze the collected opinions on the desire 
for balance in the field, the 
impact of globalization, the necessity of outreach, how to build the field, 
the physics that drives the field, and the selection of the next big machine. 
Respondents' comments follow the survey analysis in an appendix.

 



==> acknowledge2.tex <==
\section{Acknowledgments}

We thank all who have helped us in the preparation and advertisement 
of the YPP survey, including Jonathan 
Bagger, Ken Bloom, Liubo Borissov, Janet Conrad, Kevin McFarland, Paul 
Nienaber, Marv Goldberg, and Chris Quigg;  special thanks to Diana Canzone 
and Fred Ullrich of Fermilab Visual Media Services. 




==> authorlist2.tex <==
\begin{center}
\vspace*{.2 in}
{\large \bf AUTHOR LIST\\}
\vspace*{.1 in}
\end{center}

\begin{center}
  \large{\verb+ypp2000@fnal.gov+}


\vspace{0.8in}
B.~T.~Fleming$^{1}$, J.~Krane$^{2}$, G.~P.~Zeller$^{3}$,
F.~Canelli$^{4}$, B.~Connolly$^{5}$, R.~Erbacher$^{6}$, G.~T.~Fleming$^{7}$,
D.~A.~Harris$^{6}$, E.~Hawker$^{8}$, M.~Hildreth$^{9}$, B.~Kilminster$^{4}$,
S.~Lammers$^{10}$, D.~Medoff$^{11}$, J.~Monroe$^{1}$, D.~Toback$^{12}$, 
M.~Sorel$^{1}$, A.~Turcot$^{13}$, M.~Velasco$^{3}$, M.~O.~Wascko$^{14}$,
G.~Watts$^{15}$, and~E.~D.~Zimmerman$^{16}$.

\vspace{0.5in}
\noindent
$^1$Columbia University \\
$^2$Iowa State University \\
$^3$Northwestern University \\
$^4$University of Rochester \\
$^5$Florida State University \\
$^6$Fermi National Accelerator Laboratory\\
$^7$The Ohio State University\\
$^8$University of Cincinnati\\
$^9$University of Notre Dame\\
$^{10}$University of Wisconsin\\
$^{11}$University of Maryland\\
$^{12}$Texas A\&M University\\
$^{13}$Brookhaven National Laboratory\\
$^{14}$Louisiana State University\\
$^{15}$University of Washington\\
$^{16}$University of Colorado at Boulder\\

\end{center}

\newpage

==> balance2.tex <==
\section{Balance vs. Focus}

A balanced physics program at a laboratory can be achieved through several 
mechanisms; the YPP survey explores four of them.  First, an accelerator 
complex could host a range of accelerator experiments, including fixed-target
experiments, specialized collider experiments, and large multi-purpose
collider detectors. Second, two or more redundant detectors at one
facility can be built to allow several measurements of the same
quantities.  Third, more attempts could be made to balance the number
of experimentalists, theorists, and phenomenologists in the field.
Finally, facilities and resources can be shared with astrophysics experiments.
This section of the survey attempts to determine what HEP physicists are 
willing to sacrifice if diversity cannot be maintained in the face of major 
new construction and a finite budget.\\

As indicated in Figure~\ref{fig:diversity}, a majority of all
scientists believe diversity is very important in terms of the
different types of physics results they expect from the next facility.
A fixed-target program has been a natural way to achieve this
diversity at a $p\overline{p}$ machine.  A linear collider might achieve this
by having a low-energy interaction point and/or an x-ray facility,
and a muon collider by having a neutrino factory.\\

In terms of redundancy, very few physicists seem willing to rely on
a single large detector for any given analysis (Figure~\ref{fig:redundancy}). 
Despite the presumed high cost of a second multi-purpose detector, it seems
we believe the ability to verify experimental measurements is worth the 
additional expense.\\

%apparently we believe we can't afford to let inaccurate results stand 
%unchallenged.\\


\begin{figure}[ht]
\mbox{
\begin{minipage}{0.5\textwidth}
\centerline{\epsfxsize 3.0 truein \epsfbox{plots2/survey-diversity.eps}}
\vspace{-0.2in}
\caption[Should the ``next machine'' host diverse experiments and collaborations?]
        {Is it important that the ``next machine'' host a diverse (multi-physics) 
         range of experiments and collaborations?
         Recall that the solid lines indicate young physicists, and 
         dashed lines indicates tenured physicists.}
\label{fig:diversity}
\end{minipage}\hspace*{0.02\textwidth}
\begin{minipage}{0.5\textwidth}
\centerline{\epsfxsize 3.0 truein \epsfbox{plots2/survey-redundancy.eps}}   
\vspace{-0.2in}
     \caption[Is it important to have at least two detectors?]
             {If the ``next machine'' is a collider ($e^{+}e^{-},p
              \overline{p},\mu^{+}\mu^{-}$), is it important to have at 
              least two large, multipurpose detectors versus a single 
              detector?}
  \label{fig:redundancy}
\end{minipage}
}
\end{figure}

\vspace{0.1in}
Some believe that few permanent positions exist for phenomenologists relative 
to experimentalists. Comments from the survey and town meeting \cite{townmeet}
suggest a perception that undue resources are going to particular branches
of theory (e.g. string theory) at the cost of other theoretical research.
One could imagine trying to ``correct'' each perceived imbalance, or 
to continue the current free-market policy. Figure~\ref{fig:theorists} shows 
that most Americans, both young and tenured, believe it is somewhat 
important to promote a particular mix; non-Americans appear to favor 
incentives more strongly.\\

\begin{figure}[ht]
\mbox{
\begin{minipage}{0.5\textwidth}
\centerline{\epsfxsize 3.0 truein \epsfbox{plots2/survey-theorist-balance.eps}}
\vspace{-0.2in}
\caption[Is it important to balance the numbers of 
         theorists and experimentalists?]
        {Is it important to promote a balance between the numbers of 
         theorists, phenomenologists, and experimentalists?}
\label{fig:theorists}
\end{minipage}\hspace*{0.02\textwidth}
\begin{minipage}{0.5\textwidth}
\centerline{\epsfxsize 3.0 truein \epsfbox{plots2/survey-astro.eps}}   
\vspace{-0.2in}
\caption{Is it important that the HEP labs host astrophysics efforts?}
\label{fig:astro}
\end{minipage}
}
\end{figure}

\vspace{0.1in}
HEP laboratories host several astrophysics efforts, including the Sloan 
Digital Sky Survey, GLAST, and the Pierre Auger project.  Scientists feel 
it is somewhat important for this to continue, as shown in 
Figure~\ref{fig:astro}.\\

One might have expected a willingness to sacrifice redundant detectors
and small experiments in the quest for ever higher energies.  In this section,
high energy physicists have clearly stated the importance of a full physics
program at the site of the next major facility, not just the bare minimum 
required to operate the lab with a single detector at the frontier energy.  

\clearpage
\newpage








==> building2.tex <==
\section{Building the Field}

For purposes of the survey, ``building the field'' refers to increasing the
numbers and quality of physicists in HEP.  This can be accomplished
by attracting larger numbers of talented graduate students, by
retaining larger numbers of talented graduates, or both.  In this
section, we explore the reasons people come to physics, why they
might feel compelled to leave and if we are retaining enough
talent to accomplish the goals of the field.\\

In answer to the question of what most attracted them to the field,
most respondents selected ``interest in physics/science/nature'' as
their reason (Figure~\ref{fig:attracted}).  This was also the most
popular reason people have stayed (Figure~\ref{fig:stay}). 
The intellectual atmosphere and academic freedom options placed a
distant second and third, respectively. Only a few percent were attracted 
because it was ``good experience for any career path'' (i.e. fewer than the 
number that joined because they simply ``thought it was cool''), so this seems 
to be a weak selling point.

\vspace{-0.1in}
\begin{figure}[ht]
\mbox{
\begin{minipage}{0.5\textwidth}
\centerline{\epsfxsize 3.0 truein \epsfbox{plots2/survey-attracted.eps}}
\vspace{-0.2in}
\caption{What is it that \textbf{most} attracted you to HEP?}
\label{fig:attracted}
\end{minipage}\hspace*{0.02\textwidth}
\begin{minipage}{0.5\textwidth}
\centerline{\epsfxsize 3.0 truein \epsfbox{plots2/survey-stayed.eps}}   
\vspace{-0.2in}
\caption{What is the main reason you have stayed in the field so far?}
\label{fig:stay}
\end{minipage}
}
\end{figure}

\vspace{0.1in}
As shown in Figure~\ref{fig:talent}, less than 20$\%$ of all
respondents are certain that we are retaining adequate numbers of talented
physicists.  If we do indeed need to build the field, then we must
address the outward pressures that are causing HEP physicists to leave
their posts.  As shown in Figure~\ref{fig:leave}, most physicists 
believe that people leave primarily because of the lack of permanent 
positions.  Because universities employ approximately two-thirds of tenured 
scientists in the field, increased funding for university HEP might place
them in a better position to address this shortfall than the labs.\\

\begin{figure}[ht]
\mbox{
\begin{minipage}{0.5\textwidth}
\centerline{\epsfxsize 3.0 truein \epsfbox{plots2/survey-talent.eps}}
\vspace{-0.2in}
\caption[Are we retaining adequate numbers of talented physicists in HEP?]
        {Do you think we are currently retaining adequate numbers of 
         talented physicists in HEP?}
\label{fig:talent}
\end{minipage}\hspace*{0.02\textwidth}
\begin{minipage}{0.5\textwidth}
\centerline{\epsfxsize 3.0 truein \epsfbox{plots2/survey-leave.eps}}   
\vspace{-0.2in}
\caption[What most
         influences young people to leave the field?]
{What feature of the field do you think might \textbf{most} 
         influence young people to leave the field?}
\label{fig:leave}
\end{minipage}
}
\end{figure}


\vspace{0.2in}
We emphasize that Figure~\ref{fig:careerstage} in the Demographics section
indicates ample numbers of graduate students answering the survey; if we 
retain them all there certainly would be no lack of scientists for our work.  
If it is believed that the field will face a talent shortage in the future, 
then the survey results and many of the comments support one particular solution: 
create more permanent positions.

\clearpage
\newpage




==> conclusions2.tex <==
\section{Conclusions}

First and foremost, both young and tenured physicists appear to 
have similar opinions on the future course of high energy 
physics. There are, however, strong correlations 
depending on geography.\\

The survey results indicate accelerator based science is the driving force 
in HEP.  Maintaining diversity and 
balance in their work is seen as very important, but support for 
astrophysics at HEP labs is only somewhat supported.  Higgs and 
electroweak symmetry breaking are clear 
priorities, and this science requires a new facility.\\

Physicists indicated that they value 
the kind of hands-on experience that comes from being stationed at a 
laboratory.  If lab proximity becomes difficult, regional centers
might become a necessary alternative.\\

An overwhelming majority of physicists believe we are not doing enough
outreach to the funding agencies or to the general public. At least
half of these physicists would be willing to dedicate more of their
time to this effort. \\

There is some agreement that we are currently not retaining
enough young talent in the field.   The primary reason for this
is the lack of permanent positions, indicating that a lack of 
career security is the perceived force driving away young physicists.\\

Given the choice of building a linear collider (TESLA, NLC, or CLIC), 
reserving judgement for several years, or creating their own option, 
80\% of Americans and non-Americans prefer a linear collider.
Site location does not exhibit the same clear agreement: 

\begin{itemize}
     \item Non-Americans clearly do not think it is important 
           that the next machine be built in the U.S., and they
           selected the German option three to one over a U.S. option
     \item Young Americans are almost equally divided on whether there 
           should be a new linear collider in the U.S. or TESLA in Germany
     \item Tenured Americans select the U.S. option over the German
           option in a ratio of three to two
\end{itemize}

The results cannot determine how acceptable the respondents would 
find their second choice to be.\\

Given current construction and operation cost estimates, 
many countries will have to cooperate to build a new flagship facility,
and support of high energy physicists within these countries will need 
to be strong. The differences in opinion regarding the location of the 
future machine might make this necessary collaboration difficult.  More 
work is needed to forge a truly global consensus on the next machine.

\newpage


==> demographics2.tex <==
\section{Demographics}
This section summarizes the personal information of the respondents
to the YPP survey.  It was not the intention of YPP to gather
a representative sample of HEP physicists; rather, we wanted to
gather sufficient statistics from each existing demographic.
The interested analyst can re-weight the samples if desired.\\

A total of 1508 survey responses were received before the deadline. 
Another 30 responses came in after deadline, and were excluded from the sample.
More than half of the respondents (857) met the YPP definition of a young
physicist. Figure~\ref{fig:careerstage} shows the total number of
responses from each of the career stage groups.  More than 650
responses came from tenured physicists, compared to roughly 350 from
graduate students.

\begin{figure}[ht]
\centering
     \epsfysize=3.0in \epsfbox{plots2/demographics-career.eps}\vspace{-0.3in}
     \caption{Current career stage of survey respondents.}
  \label{fig:careerstage}
\end{figure}

\vspace{0.2in}
Because survey responses seemed to correlate more strongly with geography 
than with career stage, we subdivided the samples based on the respondents' 
continent of origin.  Respondents stating that they had ``grown
up'' in North America were classified as \textit{Americans}, while all others were 
classified as \textit{non-Americans} (Figure~\ref{fig:contrais}). 
To illustrate these differences, the data sample is often divided
into 4 subsets: young Americans, young non-Americans, tenured
Americans, and tenured non-Americans.  Separating the samples based on where
one currently works yields similar results, except in questions that relate most
specifically to the future of HEP in the United States.  In these instances,
separate histograms show the responses subdivided in both ways, first by
continent of origin, and then by continent on which one works.
The largest single subclass, \textit{young non-Americans}, is approximately 
$50\%$ larger than the three other subclasses (Table~\ref{table:population}).\\

\begin{figure}[ht]
\centering
     \epsfysize=3.0in \epsfbox{plots2/demographics-contrais.eps}\vspace{-0.2in}
     \caption{Continent where survey respondents grew up.}
  \label{fig:contrais}
\end{figure}

\begin{table}[ht]
\centering
   \begin{tabular}{|l|c|c|c|}\hline
                             &  Young  & Tenured  & Total  \\ \hline
 {Americans}                 & {334}   & {328}    & {662}  \\ \hline
 {Non-Americans}             & {523}   & {323}    & {846}  \\ \hline\hline
 {Total}                     & {857}   & {651}    & {1508} \\ 
\hline
   \end{tabular}
   \caption{Number of survey respondents by career stage
            and continent of origin.} 
   \label{table:population}
\end{table} 
\vspace{0.2in}

Of the 662 respondents who grew up in North America, almost all of them still 
work in North America (Figure~\ref{fig:contwork}).  In contrast, roughly 
half of the 676 European and 125 Asian respondents (including Russia and the 
Indian subcontinent) have traveled to North America to work 
(Figure~\ref{fig:contwork}).\\

Most responses came from experimentalists working in collider physics 
(Figure~\ref{fig:physwork}) at FNAL (404 responses), SLAC (168), 
DESY (192), CERN (102), or a university group (405), as depicted by 
Figure~\ref{fig:labwork}.  Responses in the ``Other'' category in Figure 5 
include 26 people from Cornell/LNS, 5 from LANL, 4 from JLAB, 3 from Kamland 
and the rest from a wide variety of institutes and research centers around the 
world. Most responses indicated work on large collaborations of more than 
200 participants (Figure~\ref{fig:collsize}).  In the survey analysis, the 
opinions of all respondents generally follow those specific to this major
constituency of collider experimentalists on large collaborations.\\

Of the 1508 respondents, only 24$\%$ (356)\footnote{In the presentation
at Snowmass, the fractions of responses from inside and outside
Snowmass were inadvertently reversed.} reported that they attended the 
Snowmass 2001 workshop, for which 1162 scientists were registered. As a 
result, this survey is predominantly representative of those who were not in
attendance at Snowmass, and hence reflects a slightly wider global distribution
of physicists (Figure~\ref{fig:labwork-atsmass}).


\begin{figure}[ht]
\mbox{
\begin{minipage}{0.5\textwidth}
\centerline{\epsfxsize 3.0 truein \epsfbox{plots2/demographics-contwork.eps}}   
\vspace{-0.2in}
\caption{On which continent do you currently work (greatest part of the 
         year)?}
\label{fig:contwork}
\end{minipage}\hspace*{0.02\textwidth}
\begin{minipage}{0.5\textwidth}
\centerline{\epsfxsize 3.0 truein \epsfbox{plots2/demographics-physwork.eps}}   
\vspace{-0.2in}
\caption{What type of physics have you been working on this year?}
\label{fig:physwork}
\end{minipage}
}
\end{figure}

\begin{figure}[hb]
\mbox{
\begin{minipage}{0.5\textwidth}
\centerline{\epsfxsize 3.0 truein \epsfbox{plots2/demographics-labwork.eps}}   
\vspace{-0.2in}
\caption{Where do you do your research (greatest part of year)?}
\label{fig:labwork}
\end{minipage}\hspace*{0.02\textwidth}
\begin{minipage}{0.5\textwidth}
\centerline{\epsfxsize 3.0 truein \epsfbox{plots2/demographics-collsize.eps}}   
\vspace{-0.2in}
\caption{How large is your current collaboration (in number of people)?}
\label{fig:collsize}
\end{minipage}
}
\end{figure}

\begin{figure}[ht]
\centering
     \epsfysize=4.0in \epsfbox{plots2/demographics-labwork-atsmass-youngold.eps}\vspace{-0.2in}
     \caption[Place where respondents currently work]
             {Place where respondents currently work separated by those who
              attended Snowmass (top) versus those who did not (bottom).}
  \label{fig:labwork-atsmass}
\end{figure}


\clearpage
\newpage









==> globalization2.tex <==
\section{The Impact of Globalization}

This section of the survey asked questions that become most relevant
if an experiment and accelerator are located far from the home
institution.  For many respondents, the questions asked here might not
draw from direct experience.  To minimize responses drawn from
conjecture, several of the questions focus on the respondents'
current situation.\\

The first question asked how frequently the respondent saw or worked
on their detector (Figure~\ref{fig:seeDet}).  Is it, in fact,
important to see your detector?  The frequency
people reported in this first question
seems quite high and might have been more informative had we asked,
``How often do you see or work on your detector for more than two hours
at a time?''  In the complementary question on the importance of
being near the detector versus near their supervisor, most selected the
detector as having the primary importance (Figure~\ref{fig:advisDet}).
We conclude that, given the choice, few physicists would prefer to work
exclusively at their home institution if they could instead work at 
the lab for a significant fraction of their time.

\begin{figure}[htp]
\mbox{
\begin{minipage}{0.5\textwidth}
\centerline{\epsfxsize 3.0 truein \epsfbox{plots2/globalization1.eps}}   
\caption{How frequently do you currently see or work on your detector?}
\label{fig:seeDet}
\end{minipage}\hspace*{0.02\textwidth}

\begin{minipage}{0.5\textwidth}
\centerline{\epsfxsize 3.0 truein \epsfbox{plots2/globalization3.eps}} 
\caption[How do you rate being near your detector versus being near your 
              supervisor?]
{In your current situation, given the choice, how do you 
              rate being near your detector versus being near your 
              advisor/supervisor?}
\label{fig:advisDet}
\end{minipage}
}
\end{figure}


The prevailing opinion is that hands-on hardware experience is
very important (Figure~\ref{fig:handsDet}).  In a future survey, 
it might be interesting to learn how much hardware work is 
enough to satisfy the need.  Likewise, one could ask 
how much analysis work is sufficient to make a well-rounded physicist.\\

The next three questions dealt, directly or indirectly, with the
concept of regional centers.  These proposed structures consist of a
facility with remote control rooms, excellent (perhaps permanent) video
conferencing, and data processing ability.  The concept of a regional
center is very new and complicated; the survey questions were not able
to explore the idea as deeply as the town meeting \cite{townmeet} at
Snowmass 2001.  Although most physicists
appear to be interested in the concept of regional centers 
(Figure~\ref{fig:rceasy}), they need to see the concept demonstrated before
they can evaluate it.  The majority of physicists want to
see national labs keep their strong roles; so if a single new frontier
facility is built, a regional center could be placed at each national
lab in the countries that do not host the facility (Figures~\ref{fig:rclocate}
and \ref{fig:uslabs}).

\begin{figure}[ht]
\mbox{
\begin{minipage}{0.5\textwidth}
\centerline{\epsfxsize 3.0 truein \epsfbox{plots2/globalization2.eps}}   
\caption{How important do you feel it is to have hands-on
              hardware experience?}
\label{fig:handsDet}
\end{minipage}\hspace*{0.02\textwidth}

\begin{minipage}{0.5\textwidth}
\centerline{\epsfxsize 3.0 truein \epsfbox{plots2/globalization4.eps}}
\vspace{0.1in}   
\caption[Should we have ``regional centers'' in the U.S.?]
{If the next machine is not located in the U.S., will the 
              quality of beams and physics results improve if we have
  	      ``regional centers'' in the U.S.?}
\label{fig:rceasy}
\end{minipage}
}
\vspace{0.2in}
\end{figure}


\begin{figure}[htp]
\mbox{
\begin{minipage}{0.5\textwidth}
\centerline{\epsfxsize 3.0 truein \epsfbox{plots2/globalization6.eps}}   
\caption{What should be the role of the U.S. national labs 
              in the next 10-25 years?}
\label{fig:uslabs}
\end{minipage}\hspace*{0.02\textwidth}

\begin{minipage}{0.5\textwidth}
\centerline{\epsfxsize 3.0 truein \epsfbox{plots2/globalization5.eps}}   
\caption[How frequently should these regional centers be distributed?]
        {How frequently should these regional centers be distributed
         relative to the current national labs?}
\label{fig:rclocate}
\end{minipage}
}
\end{figure}
      
\clearpage
\newpage


==> intro2.tex <==
\section{Introduction}

The Young Physicists' Panel (YPP) was founded in May of 2000 by Bonnie
Fleming, John Krane, and Sam Zeller  
to provide young particle physicists with a forum in which to discuss the 
future of our field.  Our first goal was to directly involve young physicists 
in the planning of the future of HEP, and to act as their conduit to 
the DOE/NSF HEPAP Subpanel on Long Range Planning for U.S. High Energy
Physics \cite{hepap}. Originally, the YPP intended to present the subpanel 
with a simple and brief document that summarized our views.  We found that 
the members of our group, and we think physicists in general, did not have a
single opinion to convey.  Our vision grew from the need to poll our own
members for their opinions, and culminated in the creation of a \textit{Survey
on the Future of HEP}, a tool to quantify the opinions of all HEP physicists 
around the globe. \\

To be most useful to the HEPAP subpanel, we created a survey with several
questions that were specific to the United States.  In keeping with our
mission, we also asked questions of particular relevance to young high
energy physicists.  Rather than limit the survey to a particular 
subsample of physicists, we opened it to all physicists to see if opinions 
differed by career stage, by laboratory, by nationality, or any other metric. 
We believe the final product provides a uniquely useful ``snapshot'' of the
field.\\

What is a ``young'' physicist? We have defined a young physicist as any 
researcher who has neither tenure nor any other permanent position in the 
field. This classification includes undergraduates, graduate 
students, postdocs, untenured faculty, and term staff; thus, ``young'' refers 
to one's sense of career security more than to one's age.

\newpage


==> method2.tex <==
\section{Methodology}


The survey questions were designed to extract maximum information with
the minimum possible bias in as short a time as possible.  Although
essay questions might seem ideal, many people are daunted by the idea
of spending hours on a well-constructed response.  We believed that
multiple choice questions would achieve a much higher yield of 
responses, and spark brief but useful essay responses as well.\\

The YPP survey questions suffered many months of invention, selection,
modification, and rejection. Essential contributions were made by Dr. Deborah 
Medoff, a statistician from the University of Maryland's School of Medicine, 
who specializes in the creation and review of surveys for psychiatric studies.
She advised us to carefully identify our event sample and refine our question 
content, in particular helping us to remove bias from leading questions in the
survey. Eventually the survey was released to external reviewers 
including several senior scientists and members of the HEPAP subpanel. \\

The survey opened on July 2, 2001 to coincide with the Snowmass
workshop -- as large a concentration of high energy physicists as one
could hope for -- and ran for two weeks.  We offered both a web-based 
version and an identical paper version. 
Advertisement at Snowmass consisted of flyers posted in the 
common areas, mention in the pamphlets for young physicists (available 
outside the main conference room), and note cards distributed by hand and 
placed in front of the common PCs in the computing center.  A single mass 
e-mail was sent to a list of young Snowmass participants compiled by the 
Young Physicists Forum steering committee \cite{ypf}.  Advertisement 
outside Snowmass was entirely electronic and targeted individual labs and the 
home institutions of YPP members.  Notices were also placed in 
D\O\ news, CDF news, and mailed to collaboration lists at SLAC, BNL, DESY, 
KEK, and several university HEP groups.\\

More than 99$\%$ of the surveys were received via the web. The
approximately 10 paper copies collected at Snowmass were entered 
into the web interface by hand. At two points during the course of the survey
we refined our advertising focus after examining demographic data: 
the fraction of young respondents and the individual lab response rates.
None of the other survey data were reviewed until three days
before the close of the survey. This practice minimized the chances 
of accidentally biasing the survey's sample pool and still allowed time to 
prepare plots and talks for presentation at the Snowmass Young Physicists'
Forum on July 17th, 2001 \cite{townmeet}. There were no additional 
advertisements after the full review. The results did not change to any 
significant degree in the final three days of the survey.\\

Responses were screened for possible duplicate submissions with a simple
script that located identical responses received within minutes of
each other from the same IP address.  The script flagged several occurrences,
in which case only a single copy of the response was retained.  With the 
exception of this filter, we relied on our colleagues to answer the survey 
only once.\\

A combination of \verb+tcsh+ and \verb+awk+ scripts converted the web 
responses into raw data files.  The raw data are available from 
\verb+http://ypp.hep.net+ 
in three formats: a .csv file for use with Excel, ntuples for {\sc Paw}, 
and a Root-tuple for the {\sc Root} analysis system.  All histograms 
in this document were generated with a standard macro file and the {\sc Paw} 
program.  This macro and its {\sc Root} analogue are available with the 
aforementioned data.  Our goal is to make these results as accessible 
as possible, so please contact us \cite{ypp} if you have special needs.\\

Most of the histograms in this document are normalized 
to yield the fraction of physicists who selected a given
response.  When two lines appear in the same histogram, the solid line 
indicates responses from young physicists, the dotted line indicates 
responses from tenured physicists.
Often, the samples are subdivided based on geography (see next section), 
yielding multiple-panel histograms.
Several histograms are not normalized, in which case the scale at the 
left is absolute.  In one instance, the sample size is dramatically reduced 
so we include the statistical error bars.\\

The figure captions contain the survey questions, either accurately reproduced
or faithfully paraphrased.  The response options, listed on the x-axis of the
histograms, are accurately reproduced where space allows and
paraphrased elsewhere.  Please refer to the original survey (included as
section 12 of this document) for the exact form of any questions 
or response options. \\

All comments from the survey are included in the long form of this document.  
They were edited for spelling and to remove names in some cases, but
are otherwise intact.  The comments, reordered into sections
by topic, should provide a good complement to the numerical
data provided by the survey. 

\newpage



==> outreach2.tex <==
\section{Outreach}

In the survey results, a clear majority believe
we are currently not doing enough outreach to either the funding agencies
(Figure~\ref{fig:outreach-congress}) or the general public
(Figure~\ref{fig:outreach-public}). In fact, physicists believe we
are doing a slightly worse job with the general public than with Congress.
These opinions on outreach hold whether you are a 
young or tenured physicist, an American or a non-American. \\


\begin{figure}[ht]
\mbox{
\begin{minipage}{0.5\textwidth}
\centerline{\epsfxsize 3.0 truein \epsfbox{plots2/outreach-congress.eps}}   
\vspace{-0.2in}
     \caption{Are we currently doing enough outreach to funding agencies?}
\label{fig:outreach-congress}
\end{minipage}\hspace*{0.02\textwidth}
\begin{minipage}{0.5\textwidth}
\centerline{\epsfxsize 3.0 truein \epsfbox{plots2/outreach-public.eps}}   
\vspace{-0.2in}
\caption{Are we currently doing enough outreach to the general public?}
\label{fig:outreach-public}
\end{minipage}
}
\end{figure}

\vspace{0.2in}
In the survey, the options should have read, ``more than enough, adequate,
not enough, or far too little.''  The third option came out as ``not nearly 
enough,'' a phrase which is not easily distinguishable from the fourth option.
From the observed results, we believe that most respondents 
interpreted the third option to lie somewhere in between options 2 and 4.\\

The survey contained a third question in the section, asking if the 
respondent would be willing to commit more time to outreach 
than they are currently.  Due to a technical error, the second and third
response options were accidentally combined, rendering the results 
less meaningful. Nonetheless, 49$\%$ (743) of all respondents said 
``yes'', they would personally be willing to dedicate more time to outreach;
the rest replied ``maybe'' or ``no''.


\clearpage
\newpage


==> physics2.tex <==
\section{Physics}

This section attempts to identify the physics that is driving HEP today.
The answer to this question should shape our decisions not only on the
next big facility but also on smaller programs, on our theoretical focus,
and on our strategies for the next 20 years. \\

Along with the clear preference for studies of Higgs and electroweak
symmetry breaking (EWSB), Figure~\ref{fig:you} also shows a broad interest 
in many other areas of physics.  Interestingly, younger scientists
find exotic searches to be more compelling than do tenured scientists.  
There are no significant variations in this plot as a function of geography.
In comparing Figures~\ref{fig:you} and \ref{fig:field}, it is clear
that despite their varied personal interests, the majority of physicists
believe Higgs/EWSB is the most important physics for the field 
to study in the coming years.\\


\begin{figure}[ht]
\mbox{
\begin{minipage}{0.5\textwidth}
\centerline{\epsfxsize 3.0 truein \epsfbox{plots2/survey-physics-you.eps}}
\vspace{-0.2in}
\caption[What physics would \textbf{you} personally find the most compelling in the future]
        {What physics would \textbf{you} personally find the most compelling 
         in the next 10-25 years?}
\label{fig:you}
\end{minipage}\hspace*{0.02\textwidth}
\begin{minipage}{0.5\textwidth}
\centerline{\epsfxsize 3.0 truein \epsfbox{plots2/survey-physics-field.eps}}   
\vspace{-0.2in}
\caption[What do you think is the most important physics for 
         the field in the future]
        {What do you think is the most important physics for 
         \textbf{the field} over the next 10-25 years?}
\label{fig:field}
\end{minipage}
}
\end{figure}

\vspace{0.2in}
Most respondents believe the most important physics does indeed require 
a major new facility (Figure~\ref{fig:newfacility}). Tenured scientists 
appear to believe this more strongly than their younger colleagues. 
Despite this perceived need, only 5$\%$ of all respondents 
listed accelerator physics as the most important physics
for the field in the future.\\

\newpage


\begin{figure}[ht]
\centering
   \epsfxsize 3.0 truein \epsfbox{plots2/survey-require-newfacility.eps}   
   \vspace{-0.2in}
   \caption{Does this science you selected require a major new facility?}
   \label{fig:newfacility}
\end{figure}

\vspace{0.2in}
Proposals for future frontier facilities exist in a number of countries
around the world.  Given the high cost to build and operate any of the proposed
large-scale machines, only one such facility (of a given kind) is 
likely to be built.  So how does one select a host country?
We specifically asked how important it is that the next new facility be in 
the U.S. (Figure~\ref{fig:newfacilityus}). While young American scientists 
appear to be more divided, most tenured American scientists think it is 
important to have a new facility in the U.S.  The overwhelming majority of 
non-Americans believe it is not important that a new facility be in the U.S.  
These results change slightly if they are subdivided based on where 
the respondent currently works rather than where they grew up 
(Figure~\ref{fig:newfacilityus-work-in-us}). In light of these responses,
the HEP community must take great care to select the location of the next 
machine in a way that results in global cooperation and shared funding,
rather than in duplicate, separate efforts.


\begin{figure}[ht]
\mbox{
\begin{minipage}{0.5\textwidth}
\centerline{\epsfxsize 3.0 truein \epsfbox{plots2/survey-require-newfacility-us.eps}}
\vspace{-0.2in}
\caption{Do you think it is important that the next new facility be 
         in the U.S.?}
\label{fig:newfacilityus}
\end{minipage}\hspace*{0.02\textwidth}
\begin{minipage}{0.5\textwidth}\vspace{0.9in}
\centerline{\epsfxsize 3.0 truein \epsfbox{plots2/survey-require-newfacility-us-working-in-us.eps}}   
\vspace{-0.2in}
\caption[Do you think it is important that the next new facility be 
         in the U.S.?]
        {Do you think it is important that the next new facility be 
         in the U.S.? Responses are now separated based on where the 
         respondent currently works and not where they grew up. Top plot 
         are those currently working in North America, bottom plot are those 
         currently not working in North America.}
\label{fig:newfacilityus-work-in-us}
\end{minipage}
}
\end{figure}


\clearpage
\newpage


==> pick2.tex <==
\section{Finding Consensus and Picking a Plan}

This section attempted to determine if the HEP community should
commit to a particular course within the next few years or wait
for more information.  In addition to plainly asking for a favored machine 
plan, this section tried to gauge the respondents' knowledge 
of each of the proposed machines, and to identify the most 
effective learning media.\\

Figure~\ref{fig:affectopinion} shows that a number of factors influenced
people's current opinions. Conversations with colleagues ranked first,
followed by current work, and workshop attendance.  Young physicists
are much less likely than tenured ones to report ``sitting and thinking'' 
as their major influence.

\begin{figure}[ht]
\centering
     \epsfysize=4.0in \epsfbox{plots2/survey-effect-opinion.eps}\vspace{-0.1in}
     \caption[What most affected your current opinion on the future options?]
             {What has most affected your current opinion(s) on the options 
              for the future of HEP?}
  \label{fig:affectopinion}
\vspace{0.2in}
\end{figure}

We asked respondents to rate their knowledge of each of the various
machine options, including TESLA (Figure~\ref{fig:tesla}), NLC and
CLIC (Figure~\ref{fig:nlc}), the VLHC (Figure~\ref{fig:vlhc}), the
neutrino factory (Figure~\ref{fig:nufact}), and the muon collider
(Figure~\ref{fig:mumu}).  Non-American physicists are more
knowledgeable about TESLA than their American counterparts, and
significantly less knowledgeable about the VLHC.\\

\begin{figure}[h]
\mbox{
\begin{minipage}{0.5\textwidth}
\centerline{\epsfxsize 3.0 truein \epsfbox{plots2/survey-know-tesla.eps}}   
\vspace{-0.2in}
\caption{How much do you know about TESLA?}
\label{fig:tesla}
\end{minipage}\hspace*{0.02\textwidth}
\begin{minipage}{0.5\textwidth}
\centerline{\epsfxsize 3.0 truein \epsfbox{plots2/survey-know-nlc.eps}}   
\vspace{-0.2in}
\caption{How much do you know about LC non-TESLA versions (i.e. NLC, CLIC)?}
\label{fig:nlc}
\end{minipage}
}
\end{figure}

\begin{figure}[h]
\centering
     \epsfysize=4.0in \epsfbox{plots2/survey-know-vlhc.eps}\vspace{-0.2in}
     \caption{How much do you know about the VLHC?}
  \label{fig:vlhc}
\end{figure}

\begin{figure}[h]
\mbox{
\begin{minipage}{0.5\textwidth}
\centerline{\epsfxsize 3.0 truein \epsfbox{plots2/survey-know-nufact.eps}}   
\vspace{-0.2in}
\caption{How much do you know about the Neutrino Factory?}
\label{fig:nufact}
\end{minipage}\hspace*{0.02\textwidth}
\begin{minipage}{0.5\textwidth}
\centerline{\epsfxsize 3.0 truein \epsfbox{plots2/survey-know-mumu.eps}}   
\vspace{-0.2in}
\caption{How much do you know about the Muon Collider?}
\label{fig:mumu}
\end{minipage}
}
\end{figure}


We also asked respondents if they felt they currently knew enough to form 
a decision. Figure~\ref{fig:decide} shows tenured physicists are slightly more
confident in their ability to decide than young physicists. The physicists who
attended Snowmass were far more confident that they had sufficient information
to decide (Figure~\ref{fig:decide_notsmass}).

\begin{figure}[h]
\mbox{
\begin{minipage}{0.5\textwidth}
\centerline{\epsfxsize 3.0 truein \epsfbox{plots2/survey-know-decide.eps}}   
\vspace{-0.3in}
\caption[Do you think you know enough to decide?]
{Do you think you know enough to form a decision and choose 
         from the various options?}
\label{fig:decide}
\end{minipage}\hspace*{0.02\textwidth}
\begin{minipage}{0.5\textwidth}
\centerline{\epsfxsize 3.0 truein \epsfbox{plots2/knowenou_not_atsmass.eps}}   
\vspace{-0.1in}
\caption[Snowmass: Do you think you know enough to decide?]
 {Respondents \textbf{at Snowmass}: ``Do you think you know enough to 
         form a decision and chose 
         from the various options''. Errors are statistical only; here, the
	 total number of responses is 356 for all four histograms combined.}
\label{fig:decide_notsmass}
\end{minipage}
}
\end{figure}


\clearpage

Finally, the respondents were asked to choose between several options
for a future flagship facility.  Using the online materials provided by the
proponents of each of the machine efforts, we identified the 
time-scales of the proposals and determined that only a few options
could begin construction within three to five years.\footnote{If one of 
the listed options requires more than
``several'' years to begin construction, or if an unlisted option becomes
viable in that time-frame, then the results would have to be interpreted
differently.}
We reasoned that
``committing'' to a plan that didn't begin construction within that
time was ostensibly the same as waiting and continuing research 
along the many branches.  The survey asked,
``if you had to choose from the following options, which one would you
pick:

\begin{itemize}
     \item A new e$^{+}$e$^{-}$ collider (TESLA,NLC,CLIC) in the U.S. soon,
           with continued research in VLHC, and muon storage ring/muon collider
           technologies.
     \item TESLA in Germany soon, with the goal of a post-LHC higher energy
           VLHC in the U.S.
     \item TESLA in Germany soon, with the goal of an eventual muon storage
           ring/muon collider in the U.S.
     \item Reserve judgment for several years, continue research.
     \item Other (specify in the comments section).''
\end{itemize}

The first option was intended to denote a linear collider that used 
unspecified technology \footnote{In hindsight, we wish we had listed JLC 
instead of CLIC, which is a longer-term project.}. The TESLA option was 
split in an attempt to glean 
additional information about machines in the U.S., resulting in options 2 
and 3. We only listed options that precluded all other options. For instance,
a $\sim$\$150M proton driver effort could exist concurrently with a 
multi-billion dollar flagship machine initiative. \\

Figure~\ref{fig:pick} shows the results.  To directly compare the location 
options, the two responses to build TESLA in Germany were summed and the 
result shown in Figure~\ref{fig:pick-sumtesla}.  Note the striking
difference between the viewpoints of Americans and non-Americans. This
difference becomes slightly more pronounced if we subdivide the responses 
based on where one currently works (Figure~\ref{fig:pick-workus}). In
the American responses, tenured scientists favor a linear 
collider in the U.S., while younger scientists are split on whether to build 
a linear collider here or TESLA in Germany. \\

Finally, we present the selections of the people that claimed to know
enough to make a decision (Figure~\ref{fig:finale_knoenou}) and those 
who were unsure or claimed not to know enough to make a decision 
(Figure~\ref{fig:finale_not_knoenou}).  It is interesting that many people
who claimed they did not know enough to make a decision still selected
an option other than ``reserve judgment''.\\

\begin{figure}[pt]
\centering
   \epsfxsize 2.6 truein \epsfbox{plots2/survey-pick.eps}
   \vspace{-0.1in}
   \caption{Which of the following machine options would you select?}
   \label{fig:pick}
\end{figure}

\begin{figure}[pb]
\mbox{
\begin{minipage}{0.5\textwidth}
\centerline{\epsfxsize 3.0 truein \epsfbox{plots2/finale.eps}}   
\vspace{-0.1in}
\caption{Which would you select, after summing TESLA options.}
\label{fig:pick-sumtesla}
\end{minipage}\hspace*{0.02\textwidth}
\begin{minipage}{0.5\textwidth}
   \epsfxsize 3.0 truein \epsfbox{plots2/finale_work_in_us.eps}   
   \vspace{-0.1in}
   \caption[Which would you select, separated by where the respondent 
            works]
{Which would you select, with responses separated by where the respondent 
            currently works instead of where they grew up.}
   \label{fig:pick-workus}
\end{minipage}
}
\end{figure}


\begin{figure}[h]
\mbox{
\begin{minipage}{0.5\textwidth}
\centerline{\epsfxsize 3.0 truein \epsfbox{plots2/finale_knoenou.eps}}   
\vspace{-0.2in}
\caption{Selections of people claiming to know enough to make a decision.}
\label{fig:finale_knoenou}
\end{minipage}\hspace*{0.02\textwidth}
\begin{minipage}{0.5\textwidth}
\centerline{\epsfxsize 3.0 truein \epsfbox{plots2/finale_not_knoenou.eps}}   
\vspace{-0.2in}
\caption[Selections of people who were unsure or claimed they do not know enough]
{Selections of people who were unsure or claimed they do not know enough to make a decision.}
\label{fig:finale_not_knoenou}
\end{minipage}
}
\vspace{0.2in}
\end{figure}

This section summarized respondents' opinions of the current machine choices.
Most physicists knew a ``fair amount'' about the current options, and most 
selected a linear collider somewhere in the world if the alternative was 
waiting for several more years to decide.  Americans tended to prefer a 
U.S. option and non-Americans strongly favored the German option.\\

\clearpage
\newpage





==> references2.tex <==
% Put all of the references here ...

\addcontentsline{toc}{section}{Bibliography}

\bibitem{hepap}
	The DOE/NSF High Energy Physics Advisory Panel created a subpanel
	to develop a long range plan for the U.S. High Energy Physics Program
       (\verb+http://hepserve.fnal.gov:8080/doe-hep/lrp_panel/index.html+).
        \\ Subpanel chairs: Jonathan Bagger and Barry Barish.

\bibitem{ypf}
	The Young Physicists Forum (YPF) Snowmass Steering Committee 
        (\verb+http://portia.fnal.gov/~bfleming/steeringcommittee.html+).

\bibitem{townmeet}
	The Young Physicists Forum (YPF) Town Meeting occured at Snowmass, 
        Tuesday, July 10, 2001 
        (\verb+http://portia.fnal.gov/~bfleming/calendar.html+).

\bibitem{ypp}
	The Young Physicists Panel (YPP) contact information is available on
        our website, \verb+http://ypp.hep.net+, also email can be sent to 
        \verb+ypp2000@fnal.gov+.




==> survey2.tex <==
\section{Survey}

The following is a complete listing of the survey questions and
possible responses as it appeared on the web. As a guide for the PAW ntuple 
and ROOT-tree (available on the web at \verb+http://ypp.hep.net+), variable 
names are listed in brackets at the end of each survey question.

\newpage

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% First Page
\vspace{-0.6in}
\begin{center}
  \Huge{Survey on the Future of HEP}
\end{center}

\rule{\textwidth}{0.02in} 

\vspace{0.3in}
This survey is geared toward members of the high energy physics community.
Please give us your opinions on the future direction of high energy
physics. Please answer honestly, as many questions as you can.\\

The survey consists of only 36 questions, mostly multiple choice.
We ask that you first fill out a brief demographics section to help
us correlate responses. All entries will remain strictly anonymous. \\
 
We kindly ask that you fill out either the web-based version of this survey
(available at \verb+http://ypp.hep.net/survey.html+) or 
the following paper version, but not both. You can place your completed survey
in any of the orange ``YPP Survey'' boxes located around Snowmass.

\vspace{0.5in}

\OliveGreen{\framebox[6.5in]{
\parbox{\reducedwidth}{\begin{center}
{\epsfxsize=6.0in \epsfbox{plots/ypp-logo3.eps}}\end{center}}}}


\vspace{0.5in}
\begin{center}
 This survey was prepared by the Young Physicists Panel (YPP). More
 information can be found at the following website:\\

 \verb+http://ypp.hep.net+
\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Demographics 
\newpage

\twocolumn
\begin{center}
  \Huge{Demographic Information}
\end{center}
\vspace{-0.1in}
\rule{3.3in}{0.02in} 

\renewcommand{\theenumi}{\arabic{enumi}}
\renewcommand{\theenumii}{\roman{enumii}}
\begin{enumerate}
   \item At what stage are you currently in your career [\verb+career+]?
     \begin{enumerate}
        \item Undergraduate 
        \item Graduate student 
        \item Postdoc
        \item Untenured faculty or term staff
        \item Tenured faculty or permanent staff
     \end{enumerate}

   \item On which continent did you grow up [\verb+contrais+]?
     \begin{enumerate}
        \item Africa
        \item Asia
        \item Australia
        \item Europe
        \item North America
        \item South America
     \end{enumerate}

   \item On which continent do you currently work greatest part of year
         [\verb+contwork+]?
     \begin{enumerate}
        \item Africa
        \item Antarctica
        \item Asia
        \item Australia
        \item Europe
        \item North America
        \item South America
     \end{enumerate}

\newpage
    \item What type of physics have you been working on this year
          [\verb+worktype+]?
     \begin{enumerate}
        \item theory
        \item fixed target experiment
        \item collider experiment ($p\overline{p}$, e$^+$e$^-$, etc.)
        \item beam research/accelerator physics
        \item astrophysics
        \item other (please specify below)
     \end{enumerate}

   \item Where do you do your research \\ greatest part of year
         [\verb+labwork+]?
     \begin{enumerate}
        \item Argonne
        \item BNL
        \item CERN
        \item DESY
        \item FNAL
        \item KEK
        \item LBL
        \item SLAC
        \item University
        \item Other (please specify in comment section below)
     \end{enumerate}

    \item How large is your current collaboration [\verb+collsize+]?
     \begin{enumerate}
        \item 1-5 people
        \item 5-20 people
        \item 20-50 people
        \item 50-200 people
        \item 200-500 people
        \item 500-1000 people
        \item more than 1000 people
     \end{enumerate}

    \item Are you attending Snowmass [\verb+atsmass+]?
     \begin{enumerate}
        \item yes
        \item no
     \end{enumerate}

    \item Additional comments:

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Balance
\cleardoublepage

\begin{center}
  \Huge{Balance vs. Focus}
\end{center}

For the following questions, we define "next machine" as the next energy \\
frontier or flagship machine. Please \\ circle one response for each of the
\\ following questions.

\rule{3.0in}{0.02in} 
   \item Is it important that the "next machine" host a diverse (multi-physics)
         range of experiments and collaborations [\verb+divnext+]?
         \begin{enumerate}
            \item very important
            \item somewhat important
            \item not important
            \item don't know/no opinion
         \end{enumerate}

   \item Is it important that the HEP labs host astrophysics efforts
         [\verb+astrnext+]?
         \begin{enumerate}
            \item very important
            \item somewhat important
            \item not important
            \item don't know/no opinion
         \end{enumerate}

   \item If the "next machine" is a collider \\ (e$^+$e$^-$, $p\overline{p}$,
         $\mu^+\mu^-$), is it important to have at least two large, 
         multi-purpose detectors versus a single detector 
         [\verb+multnext+]?
         \begin{enumerate}
            \item redundancy is very important
            \item redundancy is somewhat important
            \item redundancy is not important
            \item don't know/no opinion
         \end{enumerate}

\newpage
   \item Is it important to promote a balance \\ between the numbers of
         theorists, \\ phenomenologists, and experimentalists [\verb+prombal+]?
         \begin{enumerate}
            \item very important/mandate the mixture
            \item somewhat important/encourage a particular mixture
            \item not important/let the market decide
            \item don't know/no opinion
         \end{enumerate}

\vspace{0.2in}
   \item Additional comments on this section \\ including what HEP can support 
         given a limited budget:

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Globalization
\cleardoublepage

\begin{center}
  \Huge{The Impact of Globalization}
\end{center}

In order to best understand your \\ responses, we ask that you answer a 
number of questions on your present \\ situation. By "regional centers" 
we mean facilities that function as remote \\ virtual control rooms with 
experts present (monitoring, data acquisition, voltages, setting parameters, 
etc), with \\exceedingly good video conferencing and data processing 
capability. Please circle one response for each of the following questions.

\rule{3.0in}{0.02in} 
   \item How frequently do you currently see or work on your detector
         [\verb+seedet+]?
         \begin{enumerate}
            \item daily/weekly
            \item monthly
            \item yearly
            \item every few years
            \item N/A - don't have a detector
         \end{enumerate}
      
   \item How important do you feel it is to have hands-on hardware
         experience [\verb+handsdet+]?
         \begin{enumerate}
            \item very important
            \item somewhat important
            \item not at all important
            \item N/A - don't have a detector
         \end{enumerate}
\newpage
   \item It may be the case that your supervisor is in a different location 
         than your \\ detector. In your current situation, given the choice, 
         how do you rate being near your detector versus being near your 
         advisor/supervisor [\verb+advisdet+]?
         \begin{enumerate}
            \item detector proximity more important
            \item advisor proximity more important
            \item roughly equal in importance
            \item N/A - don't have a detector
         \end{enumerate}

   \item If the next machine is not located in the U.S., will the
         quality of beams and physics results improve if we have\\
         "regional centers" in the U.S. [\verb+rceasy+]?
         \begin{enumerate}
            \item yes
            \item no
            \item maybe
            \item don't know/no opinion
         \end{enumerate}

   \item  How frequently should these regional \\ centers be distributed
          [\verb+rclocate+]?
         \begin{enumerate}
            \item less frequently distributed than the national labs
            \item as numerous as the national labs
            \item more frequently than the national labs
            \item don't need them
         \end{enumerate}

   \item What should be the importance of the U.S. national labs 
         in 10-25 years [\verb+uslabs+]?
         \begin{enumerate}
            \item reduced role/some labs should close
            \item much the same role/current labs should persist
            \item strong role/additional labs should open
         \end{enumerate}

\vspace{0.1in}
   \item Your comments on this section, \\ including thoughts on how you might 
         envision global collaboration working:


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Outreach
\cleardoublepage

\begin{center}
  \Huge{Outreach to Influence Funding Agencies and/or the Public}
\end{center}

How important is outreach to \\ continued support of our work? Please circle 
one response for each of the \\ following questions.

\rule{3.0in}{0.02in} 
    \item Are we doing enough outreach to funding agencies, i.e. Congress
          [\verb+congoutr+]?
         \begin{enumerate}
            \item more than enough
            \item adequate
            \item not nearly enough
            \item far too little
         \end{enumerate}

    \item Are we doing enough outreach to the general public [\verb+puboutr+]?
         \begin{enumerate}
            \item more than enough
            \item adequate
            \item not nearly enough
            \item far too little
         \end{enumerate}

    \item  Would you personally be willing to \\ dedicate more of your time
           to outreach [\verb+persoutr+]?
         \begin{enumerate}
            \item yes
            \item no
            \item maybe
         \end{enumerate}

\vspace{0.2in}
    \item Your brief comments on this section and thoughts on what we
          might do \\ differently. What we might do better:

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Building the Field
\cleardoublepage

\begin{center}
  \Huge{Building the Field}
\end{center}

Your personal experience can be insightful. Please circle one response for 
each question.

\rule{2.8in}{0.02in} 
   \item What is it that \textbf{most} attracted you to HEP [\verb+attrhep+]?
      \begin{enumerate}
        \item interest in physics/science/nature
        \item strong mentor in the field 
        \item allure of working at a HEP lab
        \item intellectual atmosphere
        \item whim/it was cool
        \item nothing else is interesting
        \item salary and benefits
        \item possibility of fame
        \item enjoy hardware work
        \item enjoy software work
        \item academic freedom
        \item lifestyle/travel/hours
        \item gain valuable experience for any career choice
        \item spiritual/religious reasons
      \end{enumerate}

   \item What is main reason you have stayed in the field so far 
         [\verb+stayhep+]?
      \begin{enumerate}
        \item interest in physics/science/nature
        \item strong mentor in the field 
        \item allure of working at a HEP lab
        \item intellectual atmosphere
        \item whim/it was cool
        \item nothing else is interesting
        \item salary and benefits
        \item possibility of fame
        \item enjoy hardware work
        \item enjoy software work
        \item academic freedom
        \item lifestyle/travel/hours
        \item gain valuable experience for any career choice
        \item spiritual/religious reasons
      \end{enumerate}

   \item Do you think we are currently retaining adequate numbers 
         of talented physicists in HEP [\verb+talenhep+]?
      \begin{enumerate}
        \item yes
        \item somewhat
        \item no
        \item don't know/no opinion
      \end{enumerate}

   \item What feature of the field do you think might \textbf{most} 
         influence young physicists to leave the field [\verb+neghep+]?
      \begin{enumerate}
        \item lack of competitive salary
        \item large collaboration sizes
        \item length of time spent in grad school
        \item amount of travel required
        \item lack of permanent job \\ opportunities
        \item lack of professional environment
        \item weak or unstructured management
        \item other (please specify in comments)
        \item not an issue (don't think many will leave)
      \end{enumerate}
    
\vspace{0.2in}    
   \item Additional comments are welcome. How do we encourage talented young 
         people to do graduate work in HEP, and then stay in the field? What 
         issues facing young physicists in the future concern you the most?

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Physics
\cleardoublepage

\begin{center}
  \Huge{Physics}
\end{center}

The direction you select for the field is largely driven by the 
fundamental \\ questions you find most compelling. \\ Please circle one
response for each of the following questions.

\rule{2.8in}{0.02in} 
   \item What physics would \textbf{you} personally find most compelling in 
         the next 10-25 years [\verb+persphys+]?
      \begin{enumerate}
         \item QCD/strong interactions
         \item Higgs physics/EW symmetry \\
               breaking
         \item CP violation
         \item neutrino physics
         \item exotic particle searches
         \item accelerator physics
         \item cosmological constant/dark matter
         \item cosmic ray physics
         \item quark gluon plasma/hadronic physics
         \item other (please specify below)
      \end{enumerate}

   \item What do you think is the most important physics for \textbf{the field}
         over the next 10-25 years [\verb+fieldphy+]? 
      \begin{enumerate}
         \item QCD/strong interactions
         \item Higgs physics/EW symmetry \\
               breaking
         \item CP violation
         \item neutrino physics
         \item exotic particle searches
         \item accelerator physics
         \item cosmological constant/dark matter
         \item cosmic ray physics
         \item quark gluon plasma/hadronic physics
         \item other (please specify below)
      \end{enumerate}
\newpage
   \item Does the science you selected above \\
         require a major new facility [\verb+facphy+]?
      \begin{enumerate}
         \item yes
         \item no
         \item maybe
         \item don't know/no opinion
      \end{enumerate}
   \item If so, do you think it is important that the new facility be in
         the U.S. [\verb+facusphy+]?
      \begin{enumerate}
         \item yes
         \item no
         \item maybe
         \item don't know/no opinion
      \end{enumerate}

\vspace{0.1in}    
   \item Your additional comments on this \\ section are welcome:


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Finding Consensus
\newpage

\begin{center}
  \Huge{Finding Consensus, Picking a Plan}
\end{center}

Please circle one response for each.

\rule{2.8in}{0.02in} 

   \item What has most affected your current opinion(s) on the
         options for the future of HEP [\verb+affopin+]?
         \begin{enumerate}
              \item your advisor
              \item your current work
              \item reading
              \item talking to colleagues
              \item attending workshops/conferences
              \item attending talks
              \item joining working groups/ \\
                    performing studies
              \item sitting and thinking
              \item other
         \end{enumerate}
 
   \item How much do you know about TESLA [\verb+knowtes+]?
          \begin{enumerate}
             \item enough or alot
             \item fair amount, but need to know more           
             \item very little or nothing  
          \end{enumerate}  
   \item How much do you know about LC non-TESLA versions, i.e. NLC, CLIC
             [\verb+knowolc+]?
          \begin{enumerate}  
             \item enough or alot
             \item fair amount, but need to know more           
             \item very little or nothing  
          \end{enumerate}  
   \item  How much do you know about the VLHC [\verb+knowvlhc+]? 
          \begin{enumerate}  
             \item enough or alot
             \item fair amount, but need to know more           
             \item very little or nothing  
          \end{enumerate}  
\vspace{0.5in}
   \item  How much do you know about the \\Neutrino Factory [\verb+knownfac+]? 
          \begin{enumerate}  
             \item enough or alot
             \item fair amount, but need to know more           
             \item very little or nothing  
          \end{enumerate}
   \item  How much do you know about the Muon Collider [\verb+knowmumu+]?
          \begin{enumerate}  
             \item enough or alot
             \item fair amount, but need to know more           
             \item very little or nothing  
          \end{enumerate}  

   \item Do you think you know enough to form a decision and chose from
         the various options [\verb+knowenou+]?
         \begin{enumerate}
             \item definitely yes
             \item probably yes
             \item unsure
             \item probably no
             \item definitely no
         \end{enumerate}

   \item If you had to choose from the following options, which one would
         you pick [\verb+choose1+]?
         \begin{enumerate}
             \item a new e+e- collider (TESLA,NLC,CLIC) in the U.S. soon, 
               with continued research in VLHC and muon storage ring/muon 
               collider technologies
             \item TESLA in Germany soon, with the goal of a post-LHC
               higher energy VLHC in the U.S.
             \item TESLA in Germany soon, with the goal of an eventual muon
               storage ring/ muon collider in the U.S.
             \item reserve judgment for several years, continue research
             \item other (please specify in comment section below) 
         \end{enumerate}

\vspace{0.1in}
   \item Your comments here, please amplify on your response to the above:

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\onecolumn
\newpage




==> title2.tex <==
\begin{center}
 \Large{\verb+http://ypp.hep.net+}
\end{center}


\begin{centering}
 \vspace{0.8in}
 \textbf{\Huge The Young Physicists Panel (YPP)}\\
 \vspace{0.3in}
 \textbf{\Large presents}\\
 \vspace{0.3in}
 \textbf{\Huge Results of the Survey on the Future of HEP}\\
\vspace{0.8in}

\begin{center}
   \framebox[5.5in]{\epsfxsize=5.0in\epsfbox{plots/ypp-logo3.eps}}
\end{center}

\vspace{0.8in}
submitted to the DOE/NSF Subpanel on Long Range Planning \\
for U.S. High Energy Physics

\vspace{0.5in}
August 23, 2001


\end{centering}

